RECAP: Transparent Inference-Time Emotion Alignment for Medical Dialogue Systems

Large language models in healthcare often produce emotionally flat or opaque responses, failing to provide the transparent reasoning required for clinical trust. We present RECAP (Reflect-Extract-Calibrate-Align-Produce), an inference-time framework grounded in cognitive appraisal theory that decomposes patient input into auditable, appraisal-theoretic stages without retraining. Across multiple benchmarks and models from 8B to 120B parameters, RECAP improves alignment with human judgments, with gains inversely proportional to model scale. Intermediate outputs further reveal that models systematically underweight relational factors such as social support. In blinded evaluations, oncology fellows rated RECAP responses significantly higher than baselines with 76-88% win rates, demonstrating that principled prompting can enhance medical AI's emotional intelligence while maintaining the transparency required for clinical deployment.

==> figures/human.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.48\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    ybar,
    bar width=35pt,
    width=\textwidth,
    height=5.5cm,
    ylabel={Win Rate (\%)},
    ylabel style={font=\small},
    symbolic x coords={Human Eval, GPT-5},
    xtick=data,
    x tick label style={font=\small},
    ymin=90,
    ymax=102,
    ytick={90,92,94,96,98,100},
    ymajorgrids=true,
    grid style={gray!20},
    enlarge x limits=0.35,
    nodes near coords,
    nodes near coords style={font=\footnotesize},
    every node near coord/.append style={yshift=2pt},
    clip=false,
]
\addplot[fill=teal!70, draw=teal!80, error bars/.cd, y dir=both, y explicit] 
coordinates {
    (Human Eval, 95.7) +- (0, 2.0)  % 95.7 ± 2.0 to capture 93.8-97.8 range
    (GPT-5, 99.0)
};
\end{axis}
\end{tikzpicture}
\caption{Win rates for emotional support}
\label{fig:human-eval-winrates}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width=\textwidth, height=5.5cm, keepaspectratio]{figures/gpt_emotional_large_fonts.pdf}
\caption{GPT-5 absolute quality scores}
\label{fig:gpt5-scores}
\end{subfigure}
\caption{Emotional support evaluation of \method{} vs. Supportive Clinician baseline. (a) Human evaluators (n=2 clinicians) show 95.7\% average preference (93.8\%-97.8\% range) and GPT-5 shows 99.0\% preference for \method{}. (b) Direct quality assessment on 1-10 scale confirms superiority with \method{} scoring 8.8 vs. baseline 4.7 (p < 0.001, n=100 samples).}
\label{fig:human-eval-combined}
\end{figure*}

==> tables/clinician_dataset_samples.tex <==
\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{|p{0.22\linewidth}|p{0.73\linewidth}|}
\hline
\multicolumn{2}{|c|}{\textbf{Single-Turn Scenario: De novo HER2-positive metastatic breast cancer}} \\
\hline

\textbf{Diagnosis} &
De novo HER2-positive metastatic breast cancer with gastric/cecal involvement. \\
\hline

\textbf{Treatment plan} &
Docetaxel + trastuzumab + pertuzumab every 3 weeks; limit docetaxel to 4--6 cycles if responding, then continue trastuzumab + pertuzumab maintenance. \\
\hline

\textbf{Narrative} &
A 60-year-old grandmother who has always held the family together. She has lost 30 lb over three months and recently learned the thickening in her stomach and colon represents metastatic breast cancer. She fears losing her identity to her grandchildren. \\
\hline

\textbf{Representative question} &
\emph{``Everyone keeps saying this plan is palliative. How do I balance hope with honesty so my family doesn't think I'm giving up?''} \\
\hline
\end{tabular}

\caption{Representative synthetic patient question used in our clinician-led evaluation, shown with diagnosis, treatment plan, and narrative context.}
\label{tab:scenario}
\end{table}


==> tables/clinician_multi-turn_sample.tex <==
\begin{table}[ht] \centering \footnotesize \begin{tabular}{|p{0.22\linewidth}|p{0.73\linewidth}|} \hline \multicolumn{2}{|c|}{\textbf{Multi-Turn Scenario: Stage IIA Classical Hodgkin Lymphoma}} \\ \hline \textbf{Diagnosis} & Stage IIA classical Hodgkin lymphoma \\ \hline \textbf{Treatment plan} & ABVD chemotherapy every 2 weeks for 2--4 cycles with response-adapted PET imaging. \\ \hline \textbf{Patient persona} & 20-year-old first-generation college student. High-achiever, pressured, dutiful. Knowledgeable about "chemo brain" and cognitive effects. Core belief: \emph{"I cannot fail. My parents sacrificed everything for me. Taking a break is not an option."} \\ \hline \textbf{Hidden goals} & Refuse to take a semester off; seek strategies to study through chemotherapy-related cognitive effects. \\ \hline \textbf{Opening statement} & \emph{"I finally made the Dean's List. I can't take a semester off. My parents worked too hard for me to be here."} \\ \hline \end{tabular} \caption{Representative multi-turn synthetic scenario used in clinician-led evaluation. The patient persona and hidden goals guide conversational evolution across 3 turns as the patient responds to system output.} \label{tab:multiturn_scenario} \end{table}

==> tables/human_eval_sample.tex <==
\begin{table}[!t]
\centering
\small
\begin{tabular}{|p{0.22\linewidth}|p{0.72\linewidth}|}
\hline
\multicolumn{2}{|c|}{\textbf{Scenario S1}} \\ \hline

$\rightarrow$ \textbf{Diagnosis} &
De novo HER2-positive metastatic breast cancer with gastric/cecal involvement \\ \hline

$\rightarrow$ \textbf{Treatment plan} &
Docetaxel + trastuzumab + pertuzumab IV every 3 weeks; limit docetaxel to $\sim$4--6 cycles if responding, then continue trastuzumab + pertuzumab maintenance \\ \hline

$\rightarrow$ \textbf{Narrative} &
I’m a 60-year-old grandmother who has always held the family together. I’ve lost 30 lb in three months and learned the thick\ldots{} already spread. My team recommends docetaxel with trastuzumab and pertuzumab. I’m afraid of losing who I am to my grandkids. \\ \hline

$\rightarrow$ \textbf{Question} &
``Everyone keeps saying this plan is palliative. How do I balance hope with honesty so my family doesn’t think I’m giving up?'' \\ \hline
\end{tabular}
\caption{Sample item fields for one synthetic scenario used in clinician-led evaluation.}
\label{tab:sample_item_fields}
\end{table}


==> tables/seceu_table.tex <==

% \begin{table}[!t]
% \centering
% \footnotesize
% \setlength{\tabcolsep}{3pt}      % default ~6pt; tighten cols
% \renewcommand{\arraystretch}{1.05}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lccccccccc@{}}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{3}{c}{Llama-3.1-8B-Instruct} & \multicolumn{3}{c}{openai-oss-20B} & \multicolumn{3}{c}{openai-oss-120B} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
% & EQ\(\uparrow\) & SECEU\(\uparrow\) & Pattern Sim.\(\uparrow\) & EQ\(\uparrow\) & SECEU\(\uparrow\) & Pattern Sim.\(\uparrow\) & EQ\(\uparrow\) & SECEU\(\uparrow\) & Pattern Sim.\(\uparrow\) \\
% \midrule
% zero-shot prompting           & $58.31_{\pm3.89}$ & $5.075_{\pm0.199}$ & $0.236_{\pm0.034}$ & -- & -- & -- & $110.49_{\pm2.16}$ & $2.215_{\pm0.118}$ & $0.314_{\pm0.101}$ \\
% emotion prompt priming        & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% supportive clinician persona  & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% EmoBIRD                       & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
% \bottomrule
% \end{tabular}
% }
% \caption{SECEU results (higher is better). Values are mean\(_{\pm\mathrm{sem}}\). Dashes indicate not measured/available.}
% \label{tab:seceu}
% \end{table}
% % 
